Imperfect Visual Verification for Code Edition : A Case Study on TikZ

LLMs have significantly advanced code generation, enabling the synthesis of functional programs. While recent systems achieve strong performance on many coding benchmarks, tasks involving programs such as TikZ that generate visual artifacts remain challenging, in particular on visual code customization. Unlike generation from scratch, customization requires localized, semantics-preserving edits: the model must locate relevant code, modify it according to the instruction, and preserve the remaining structure and rendering. Approaches based on post-hoc iterative refinement/correction where a verifier provides feedback to guide corrections, have shown promise. However, in the case of programs with a visual outcome such as in TikZ, where correctness is harder or likely impossible to formalize and evaluate automatically, deterministic verifiers do not exist. Hence, developers can only rely on imperfect verifiers. In this paper, we conduct an empirical study to answer:to what extent can iterative refinement remain effective when the verifier itself is unreliable?} We use TikZ as a focused case study that isolates the core difficulties of the problem (weak code structure, fine-grained visual semantics, and difficult feature localization) in a controlled and challenging setting. We define visual code customization as an iterative editing problem with an imperfect oracle, and introduce a framework for analyzing such iterative refinements. We conduct a large-scale study and evaluate multiple LLM-based and tool-augmented visual verifiers within iterative refinement pipelines, and perform extensive manual annotation of refinement trajectories to assess verifier behavior and feedback quality. Our findings show that even imperfect verifiers can determine with moderate accuracy whether visual instructions are applied to code, achieving F1-scores up to 0.815. Feedback improves iterative refinement, especially for weaker models, adding 11--20 perfect customizations for Qwen3-vl-30b-a3b-Instruct, while stronger models like Gemini-3 gain fewer improvements (+5) but benefit more from accurate verification that prevents premature acceptance. Feedback is effective only when it precisely identifies image issues, provides actionable guidance, addresses all relevant problems, and remains grounded in the original instruction.

==> figures/additional_figures.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{imported_figures/avg_score_step.png}
   \caption{
       Average human score per step per Verifier.
   }
    \label{figure:avg_score_step}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{imported_figures/avg_sverifier_core_step.png}
   \caption{
       Average Verifier score per step per Verifier.
   }
    \label{figure:avg_ver_score_step}
\end{figure*}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{imported_figures/avg_bump_score.png}
   \caption{
       Average bump of the score per step per Verifier.
   }
    \label{figure:avg_bump_score_step}
\end{figure}

==> former_texts/dataset_creation.tex <==

\section{Dataset Creation}


 \begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{Figures/dataset_creation.drawio.png}
   \caption{
       Dataset Creation Workflow. 
   }
    \label{fig:dataset_creationv0}
\end{figure*}
 \begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{Figures/ds_creation.drawio.png}
   \caption{
       Dataset Creation Workflow v2. 
   }
    \label{fig:dataset_creation}
\end{figure*}


Our goal was to create a dataset that would contain an instruction, along with correct and incorrect code customizations. To achieve this, we used our previous dataset VTikz\cite{reux_llm_2025}, which was the foundation for the benchmark of the same name. The goal of this dataset was to evaluate LLMs on the customization task itself, and it contained the necessary data for us to construct a new dataset VeriTikZ.

We decided to use three of the feature from this previous dataset to create VeriTikZ: the \textit{initial code}, \textit{customization instruction} and \textit{parameterized code}.

% define parameterized code
A parameterized code is a TikZ code that encompass as much possible correct solutions of a customization as possible, it achieves so using a set of statements, for example \textit{Range},\textit{Rangei}, or \textit{Choice}. These statements allows the VTikZ benchmark to compare a generated solution to a parameterized solution, by checking that the values positioned at the statements are within a range, or within a set of choices. That way, multiple shades of Red, of multiple positions can be encompassed with a parameterized code. The statement are defined as followed: ranges(lower, higher, default), rangei(value, interval) and choice([A,B,C,...], default), and are added within the parameterized code.

Our dataset is based on this previous dataset and uses the parameterized solutions to create new data, the dataset creation workflow in shown in \cref{fig:dataset_creation}. In the following section, each step of the dataset creation is explained.

\paragraph{\textbf{Data generation from existing parameterized solution}}
First, the parameterized solutions are used to create new correct and incorrect solutions. 
The correct solutions are created by simply taking the default value for each statement, while each incorrect solution is generated by taking values outside the correct set of values for 2 random statements, and the default one otherwise, essentially creating \(\binom{n_s}{2}\) incorrect solutions, with $n_s$ the number of statements.
In order to increase the difference between correct and incorrect solutions, a random modification is applied to each of these incorrect solution, these modifications include color switch, rotation, number changes, scaling, position tweaking, and node swaps. Some parameterized solutions however do not contain any statement, in that case, 5 random modifications are applied. This first data generation gives us 2286 solutions, with 140 correct and 2146 incorrect ones.

\paragraph{\textbf{Clip filtering}}
%The first filtering steps consisted of removing the non compilable codes and deduplicating,
 To ensure that an incorrect solution generated is not too similar to the perfect solutions, we computed the clip similarity between each incorrect solution and a theoretically perfect solution, and kept only the incorrect one which had a clip similarity under 0.97. resulting in 140 correct and 1502 incorrect solutions.

\paragraph{\textbf{Final Selection}}
Finally, for each correct solution, we selected at most 3 randomly incorrect solutions, finally resulting in 93 correct solutions for 214 incorrect ones.

==> imported_figures/AUC_fixed.tex <==
\begin{tabular}{l|rrr}
\toprule
Generator & Agentic Vision & Precise Score & Segmentation-Tool Verifier \\
\midrule
google/gemini-3-flash-preview & 0.690 & 0.856 & 0.503 \\
qwen/qwen3-vl-30b-a3b-instruct & 0.948 & 0.860 & 0.704 \\
\bottomrule
\end{tabular}


==> imported_figures/AUC_llm.tex <==
\begin{tabular}{ll|rrrr}
\toprule
Verifier Model & Generator & Text & Text+Visual & Visual & Visual Property \\
\midrule
Gemini Model & google/gemini-3-flash-preview & 0.544 & 0.704 & 0.752 & 0.688 \\
Gemini Model & qwen/qwen3-vl-30b-a3b-instruct & 0.881 & 0.880 & 0.855 & NaN \\
\midrule
Qwen Model & qwen/qwen3-vl-30b-a3b-instruct & NaN & NaN & NaN & 0.812 \\
\bottomrule
\end{tabular}

==> imported_figures/PR_AUC_fixed.tex <==
\begin{tabular}{l|rrr}
\toprule
Generator & Agentic Vision & Precise Score & Segmentation-Tool Verifier \\
\midrule
google/gemini-3-flash-preview & 0.846 & 0.885 & 0.659 \\
qwen/qwen3-vl-30b-a3b-instruct & 0.731 & 0.718 & 0.514 \\
\bottomrule
\end{tabular}


==> imported_figures/PR_AUC_llm.tex <==
\begin{tabular}{ll|rrrr}
\toprule
Verifier Model & Generator & Text & Text+Visual & Visual & Visual Property \\
\midrule
Gemini Model & google/gemini-3-flash-preview & 0.836 & 0.846 & 0.841 & 0.774 \\
Gemini Model & qwen/qwen3-vl-30b-a3b-instruct & 0.678 & 0.662 & 0.652 & NaN \\
\midrule
Qwen Model & qwen/qwen3-vl-30b-a3b-instruct & NaN & NaN & NaN & 0.484 \\
\bottomrule
\end{tabular}

==> sections/dataset.tex <==
Our previous dataset \textit{VTikZ} contains 100 examples of code customization, the latest evaluation with GPT 5.2 and Gemini 3 showed that they could respectively achieve 52 and 66 customization. In this work, our goal is to evaluate the iterative refinement process, hence we selected 37 out of the hundred solutions that were generally not achieved by any of the models.
\TODO{more details}

==> sections/discussion.tex <==
\paragraph{Post-Hoc Iterative Refinement and Visual Code Customization}
Stepping back from the research questions, our results more generally show that post-hoc iterative refinement improves performance in the context of TikZ code customization. It appears to be a promising approach to bridge modalities and enhance LLM capabilities. Our experiments also indicate that several factors can further improve the refinement loop, notably better scoring mechanisms and higher-quality feedback.

\paragraph{Verifiers' Quality Dimensions}
Designing an effective verifier requires attention to two key dimensions. First, the quality of the classification: a verifier must be precise and should only terminate the iteration process when the customization is correctly and fully applied. Second, the quality of the feedback, which must be \textbf{precise}, \textbf{guiding}, \textbf{complete}, and \textbf{non-forgetful} with respect to the instruction. A verifier satisfying these properties is expected to significantly improve the effectiveness of iterative refinement.

\paragraph{Performance of the segmentation-based approach}
The underwhelming performance of this approach can be attributed to three main factors. First, the method relies on the segmentation capabilities of \textit{gemini-2.5-flash}, which can be unreliable, particularly for images such as diagrams. Second, the feedback produced by the approach may be overly mechanistic, making it more difficult for the generator to interpret and apply effectively. Finally, the generated Python code verifies whether the expected modifications have been applied to the image, but does not ensure that no unintended changes have been introduced, ignoring incorrect alterations.
%I might remove it I think





==> sections/task_definition.tex <==
In order to tackle this \textit{Verifier Problem}, we introduce the tasks of Assessment of Visual Instruction Application on Code, and Visual Feedback Generation. 

The first task aims at evaluating the capabilities of a Verifier at assessing how well a generated solution satisfies an instruction. It can be described as a regression problem, in which the inputs are the \textit{instruction}, the \textit{Initial Code}, and the \textit{Customized Code}, and the output is a score from 0 to 1 (0: not applied, 1: perfectly applied). 

The second task concerns feedback, by considering the following fact better feedback will guide the generative component toward better solutions, and by using the quality of the solutions as a proxy, we can assess the quality of the feedback. The complete evaluation protocol is detailed in \Cref{sec:eval_methodo} 

==> tables/pr_auc_scores.tex <==
\begin{table*}[t]
%\renewcommand{\arraystretch}{1.1}
\centering
%\setlength{\tabcolsep}{4pt}
\caption{PR-AUCs for each verifier/generative pairs for llm verifiers}
\label{tab:pr_auc_scores_llm}
\resizebox{\linewidth}{!}{
\input{imported_figures/PR_AUC_llm}
}
\end{table*}

\begin{table*}[t]
%\renewcommand{\arraystretch}{1.1}
\centering
%\setlength{\tabcolsep}{4pt}
\caption{PR-AUCs for each verifier/generative pairs for fixed verifiers}
\label{tab:pr_auc_scores_fixed}
\resizebox{\linewidth}{!}{
\input{imported_figures/PR_AUC_fixed}
}
\end{table*}


==> tables/roc_auc_scores.tex <==

%\renewcommand{\arraystretch}{1.1}
\begin{table*}
\centering
%\setlength{\tabcolsep}{4pt}
\caption{ROC-AUCs for each verifier/generative pair for llm verifiers}
\label{tab:roc_auc_scores_llm}
\resizebox{\linewidth}{!}{
\input{imported_figures/AUC_llm}
}
\end{table*}

%\renewcommand{\arraystretch}{1.1}
\begin{table*}
\centering
%\setlength{\tabcolsep}{4pt}
\caption{ROC-AUCs for each verifier/generative pair for fixed verifiers}
\label{tab:roc_auc_scores_fixed}
\resizebox{\linewidth}{!}{
\input{imported_figures/AUC_fixed}
}
\end{table*}

